Advances in Hyperspectral Image Classification: Earth monitoring with statistical learning methods

Hyperspectral images show similar statistical properties to natural grayscale or color photographic images. However, the classification of hyperspectral images is more challenging because of the very high dimensionality of the pixels and the small number of labeled examples typically available for learning. These peculiarities lead to particular signal processing problems, mainly characterized by indetermination and complex manifolds. The framework of statistical learning has gained popularity in the last decade. New methods have been presented to account for the spatial homogeneity of images, to include user's interaction via active learning, to take advantage of the manifold structure with semisupervised learning, to extract and encode invariances, or to adapt classifiers and image representations to unseen yet similar scenes. This tutuorial reviews the main advances for hyperspectral remote sensing image classification through illustrative examples.

==> 02_standard.tex <==

\section{Standard Regularized image classification}\label{sec:robust}

%Hyperspectral images are rich and informative, but also increase significantly the dimensionality of data. 
Before HSI, most of the models used in remote sensing were parametric, such as Gaussian Maximum Likelihood (GML) or Linear Discriminant Analysis (LDA). These methods, based on the estimate of the covariance matrix, were successful when dealing with early multispectral images, whose dimensionality was usually comprised between four and ten bands. HSI changed the rules, as the dimensionality of the pixel representation raised to hundreds. Standard parametric methods became either unfeasible or unreliable, since estimating the class-covariance matrices require many labeled samples, which are usually not available. For that reason, research turned to regularized approaches, trying to limit the model complexity in the ill-posed situation of high-dimension and limited number of samples.

\vspace{-0.25cm}\subsection{Regularized parametric approaches.} %A first way to proceed is to add a regularizer to one of the traditional parametric methods, to force the sample covariance matrix toward a simpler, more stable matrix. 
Hyperspectral covariance matrices are typically conditioned via Tikhonov's regularization, $\hat{\Sigma} = \Sigma + \lambda {\Omega}$. Standard ridge reduces to ${\Omega} = {I}$. If ${\Omega} = {\beta}^\top {I}{\beta}$, where ${\beta}$ are the coefficients of optimal scoring of samples, reduces to {\em penalized discriminant analysis}~\cite{Yu99}, which %\cite{Hastie95}
downweights samples whose regression coefficients vary locally. %Using ${\Omega} = {I} - {VV}^\top$, where ${V}$ is %an orthogonal %%% THIS MUST BE WRONG: IF V IS ORTHOGONAL VV'=I
%a projection matrix to a $k$ subspace, %reducing dimensionality from $d$ to $k$ dimensions, 
%corresponds to 
Alternatively, one can perform classification in a subspace of reduced dimensionality by using ${\Omega} = {I} - {VV}^\top$, where $V$ is a projection matrix to that subspace~\cite{Jensen10}. Other strategies based on committees of classifiers trained on spectral subsets of HSI have also been proposed to attain more robust covariance estimates in LDA models~\cite{Prasad08}. % and boost final performances through decision function of the spectral views on the problem~\cite{Prasad08}.  
Finally, standard and more advanced forms of regularization are reviewed in~\cite{Bandos09}.

\vspace{-0.25cm}\subsection{Regularized nonparametric approaches.} Although successful, parametric models still rely on the assumption of normality of the class conditional PDFs. Due to the complexity of HSI, such assumption rarely holds, which encouraged research towards non-parametric models, not making any assumption on the distribution underlying the data. %However, nonparametric models are related to a strong increase of the models' parameters (typically, there are at least as many parameters as there are datapoints) and therefore placed the search for regularized solutions as a priority. % THIS IS NOT AT ALL TRUE: ACTUALLY, ONLY KERNEL METHODS FOLLOW THIS STATEMENT; NNETS OR TREES OR BOOSTING OR TYPICALLY ARE SPARSE NONPARAMETRIC MODELS...
In the last decade, SVM has become the most widely used method in HSI classification research~\cite{CampsValls05,CampsValls09}. Unlike other nonparametric approaches, such as regularized RBF networks, SVM naturally implements regularization through the concept of maximum margin: maximizing the linear separability between classes is equivalent to minimize the $\ell_2$-norm of model weights %, $\w$, 
used as regularizer. %, $\Omega=\|\w\|_2^2$. 
%is sparse and regularized by nature, since it includes in its optimization a $\ell_2$ norm regularizer of the model parameters $\mathbf{w}$, minimizing the energy of the data used and forcing smooth solutions~\cite{CampsValls05}. The problem is composed by two competing terms
%$${\mathcal L}_{reg}(x,y,f(x)) = {\mathcal L}_{emp}(f(x),y) + \lambda~||\mathbf{w}||^2_l,$$
%\begin{align}
%\min_{\w,\xi} C\sum_{i=1}^n\xi_i +& ||\w||^2_2\\
%\nonumber \text{s.t. } & y_i(\langle\w,x_i\rangle+b)\geq 1-\xi_i \text{, } \forall i, \xi_i \geq 0
%\end{align}
%The left term corresponds to the minimization of the empirical error (loss) and the right term is the SLT regularizer controlling the flexibility of the model. Using Lagrange multipliers, the final decision function is of the form 
%\begin{equation}
%y^* = f(\x^*) = sign\Big(\sum_{i=1}^n\alpha_iy_i\langlex_i , \x^*\rangle + b\Big)
%\label{eq:predSVM}
%\end{equation}
%where $\alpha_i$ are the SVM coefficients and are non-zero only for a small amount of training points (called the \emph{support vectors}). %For this reason, SVM solution is sparse.

Despite the elegance and simplicity of a nonparametric solution, SVM still provides only a linear classifier. % of type $f(\x^*) = \langle\w,\x^*\rangle + b$. 
When confronted to HSI, the linear SVM is still suboptimal since %, even if regularized, 
it does not provide nonlinear boundaries among the classes. A solution to this problem was found by SLT: the structural risk minimization principle~\cite{Vapnik98} states that it is easier to learn with a simple classifier in a higher dimensional space $\mathcal{H}$, than working in the original space $\mathcal{X}$ with a complex method. The difficulty %to apply this principle 
resides in projecting the samples $x$ into the higher dimensional space $\mathcal{H}$ using a mapping function $\phi(\cdot)$ since  there are infinitely many possible functions. %To do this, a characteristic of the decision function of Eq.~\eqref{eq:predSVM} is used: the SVM solution only depends on pairwise dot products (similarities) between each training sample and the point to predict, $\langle x_i,x^*\rangle$. The feature vectors are not used as such. 
The reproducing kernel properties gives the solution here: one only has to express model weights as a linear combination of examples in ${\mathcal H}$, and then replace the appearance of the dot products between mapped samples with a reproducing kernel function $K(x_i,x^*) = \langle \phi(x_i), \phi(x^*)\rangle_{\mathcal{H}}$ that works with input data points and represents the similarity between the samples in $\mathcal{H}$. Hence one can solve nonlinear problems by solving optimal linear classifiers in an appropriate higher dimensional vector space {\em implicitly}. %the method becomes nonlinear and performs linear separation in $\mathcal{H}$, which corresponds to a nonlinear separation in $\mathcal{X}$. This is called the \emph{kernel trick} and made the success of SVM, 
The SVM then allows to perform nonlinear classification without increasing the number of parameters, and keeps the elegant regularized formulation of the linear case.

%As for the LDA case, taking advantage of the block-diagonal structure of the covariance matrix to construct an ensemble of weak SVM classifiers boosts the performance~\cite{Waske10}.





==> abstract.tex <==
%!TEX root = fullpaper.tex
Hyperspectral images show similar statistical properties to natural grayscale or color photographic images. However, the classification of hyperspectral images is more challenging because of the very high dimensionality of the pixels and the small number of labeled examples typically available for learning. \blue{These peculiarities lead to particular signal processing problems, mainly characterized by indetermination and complex manifolds. %For these reasons, recent hyperspectral image classification research has been strongly influenced by the field of statistical inference. 
The framework of statistical learning has gained popularity in the last decade. New methods have been presented to account for the spatial homogeneity of images, to include user's interaction via active learning, to take advantage of the manifold structure with semisupervised learning, to extract and encode invariances, or to adapt classifiers and image representations to unseen yet similar scenes. 
%The design of a suitable regularized functional has led to the successful solution of many hyperspectral image classification problems. 
This tutuorial reviews the main advances for hyperspectral remote sensing image classification through illustrative examples. }% for each particular problem setting.

